Gravitational ABJ Anomaly, Stochastic Matter Production, and Leptogenesis

Partially chiral stochastic gravitational wave backgrounds can arise from various processes in the early Universe. The gravitational ABJ anomaly links the chirality of the gravitational field to the chiral fermions, resulting in the stochastic generation of fermionic matter in the radiation era. We show that this mechanism can account for the entire dark matter relic density and discuss its potential as a leptogenesis scenario to explain the observed matter-antimatter asymmetry in the Universe. Remarkably, this letter reveals that even if gravitational waves become unpolarized later, their temporary chirality during their generation process leaves a lasting imprint on the fermionic matter, preserved as a quantum remnant.

==> ref.tex <==
@article{Ford:1986sy,
    author = "Ford, L. H.",
    title = "{Gravitational Particle Creation and Inflation}",
    reportNumber = "TUTP-86-8",
    doi = "10.1103/PhysRevD.35.2955",
    journal = "Phys. Rev. D",
    volume = "35",
    pages = "2955",
    year = "1987"
}

@article{Planck:2015fie,
    author = "Ade, P. A. R. and others",
    collaboration = "Planck",
    title = "{Planck 2015 results. XIII. Cosmological parameters}",
    eprint = "1502.01589",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1051/0004-6361/201525830",
    journal = "Astron. Astrophys.",
    volume = "594",
    pages = "A13",
    year = "2016"
}



@article{Maleknejad:2012fw,
    author = "Maleknejad, A. and Sheikh-Jabbari, M. M. and Soda, J.",
    title = "{Gauge Fields and Inflation}",
    eprint = "1212.2921",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "IPM-P-2012-049, KUNS-2430",
    doi = "10.1016/j.physrep.2013.03.003",
    journal = "Phys. Rept.",
    volume = "528",
    pages = "161--261",
    year = "2013"
}

@article{Maleknejad:2014wsa,
    author = "Maleknejad, Azadeh",
    title = "{Chiral Gravity Waves and Leptogenesis in Inflationary Models with non-Abelian Gauge Fields}",
    eprint = "1401.7628",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevD.90.023542",
    journal = "Phys. Rev. D",
    volume = "90",
    number = "2",
    pages = "023542",
    year = "2014"
}

@article{Caldwell:2017chz,
    author = "Caldwell, R. R. and Devulder, C.",
    title = "{Axion Gauge Field Inflation and Gravitational Leptogenesis: A Lower Bound on B Modes from the Matter-Antimatter Asymmetry of the Universe}",
    eprint = "1706.03765",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.97.023532",
    journal = "Phys. Rev. D",
    volume = "97",
    number = "2",
    pages = "023532",
    year = "2018"
}

@article{Dimastrogiovanni:2012ew,
    author = "Dimastrogiovanni, Emanuela and Peloso, Marco",
    title = "{Stability analysis of chromo-natural inflation and possible evasion of Lyth\textquoteright{}s bound}",
    eprint = "1212.5184",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "UMN-TH-3129-12",
    doi = "10.1103/PhysRevD.87.103501",
    journal = "Phys. Rev. D",
    volume = "87",
    number = "10",
    pages = "103501",
    year = "2013"
}

@article{Komatsu:2022nvu,
    author = "Komatsu, Eiichiro",
    title = "{New physics from the polarized light of the cosmic microwave background}",
    eprint = "2202.13919",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1038/s42254-022-00452-4",
    journal = "Nature Rev. Phys.",
    volume = "4",
    number = "7",
    pages = "452--469",
    year = "2022"
}

@article{Adshead:2013qp,
    author = "Adshead, Peter and Martinec, Emil and Wyman, Mark",
    title = "{Gauge fields and inflation: Chiral gravitational waves, fluctuations, and the Lyth bound}",
    eprint = "1301.2598",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevD.88.021302",
    journal = "Phys. Rev. D",
    volume = "88",
    number = "2",
    pages = "021302",
    year = "2013"
}

@article{Alexander:2018fjp,
    author = "Alexander, Stephon and McDonough, Evan and Spergel, David N.",
    title = "{Chiral Gravitational Waves and Baryon Superfluid Dark Matter}",
    eprint = "1801.07255",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1088/1475-7516/2018/05/003",
    journal = "JCAP",
    volume = "05",
    pages = "003",
    year = "2018"
}

@article{Maleknejad:2016dci,
    author = "Maleknejad, Azadeh",
    title = "{Gravitational leptogenesis in axion inflation with SU(2) gauge field}",
    eprint = "1604.06520",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1088/1475-7516/2016/12/027",
    journal = "JCAP",
    volume = "12",
    pages = "027",
    year = "2016"
}



@article{Kharzeev:2013ffa,
    author = "Kharzeev, Dmitri E.",
    title = "{The Chiral Magnetic Effect and Anomaly-Induced Transport}",
    eprint = "1312.3348",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1016/j.ppnp.2014.01.002",
    journal = "Prog. Part. Nucl. Phys.",
    volume = "75",
    pages = "133--151",
    year = "2014"
}

@article{Hawking:1975vcx,
    author = "Hawking, S. W.",
    editor = "Gibbons, G. W. and Hawking, S. W.",
    title = "{Particle Creation by Black Holes}",
    doi = "10.1007/BF02345020",
    journal = "Commun. Math. Phys.",
    volume = "43",
    pages = "199--220",
    year = "1975",
   % note = "[Erratum: Commun.Math.Phys. 46, 206 (1976)]"
}

@article{Maleknejad:2024hoz,
    author = "Maleknejad, Azadeh and Kopp, Joachim",
    title = "{Weyl Fermion Creation by Cosmological Gravitational Wave Background at 1-loop}",
    eprint = "2406.01534",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "KCL-PH-TH/2024-33, CERN-TH-2024-079, MITP-24-054",
    month = "6",
    year = "2024"
}

@article{Adshead:2015pva,
    author = "Adshead, Peter and Giblin, John T. and Scully, Timothy R. and Sfakianakis, Evangelos I.",
    title = "{Gauge-preheating and the end of axion inflation}",
    eprint = "1502.06506",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1088/1475-7516/2015/12/034",
    journal = "JCAP",
    volume = "12",
    pages = "034",
    year = "2015"
}

@article{Fu:2024ipa,
    author = "Fu, Chengjie and Chen, Chao and Wang, Yi",
    title = "{Bridging inflation and reheating: chiral gravitational waves from aHz to GHz}",
    eprint = "2410.06636",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    month = "10",
    year = "2024"
}

@article{He:2021kah,
    author = "He, Yutong and Roper Pol, Alberto and Brandenburg, Axel",
    title = "{Leading-order nonlinear gravitational waves from reheating magnetogeneses}",
    eprint = "2110.14456",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "NORDITA-2021-080",
    month = "10",
    year = "2021"
}

@article{Maleknejad:2024ybn,
    author = "Maleknejad, Azadeh and Kopp, Joachim",
    title = "{Gravitational Wave-Induced Freeze-In of Fermionic Dark Matter}",
    eprint = "2405.09723",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "KCL-PH-TH/2024-28, CERN-TH-2024-061, MITP-24-050",
    month = "5",
    year = "2024"
}

@article{Maleknejad:2023nyh,
    author = "Maleknejad, Azadeh",
    title = "{Photon chiral memory effect stored on celestial sphere}",
    eprint = "2304.05381",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "CERN-TH-2023-052",
    doi = "10.1007/JHEP06(2023)193",
    journal = "JHEP",
    volume = "06",
    pages = "193",
    year = "2023"
}


@article{Kahniashvili:2020jgm,
    author = "Kahniashvili, Tina and Brandenburg, Axel and Gogoberidze, Grigol and Mandal, Sayan and Roper Pol, Alberto",
    title = "{Circular polarization of gravitational waves from early-Universe helical turbulence}",
    eprint = "2011.05556",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "NORDITA-2020-102",
    doi = "10.1103/PhysRevResearch.3.013193",
    journal = "Phys. Rev. Res.",
    volume = "3",
    number = "1",
    pages = "013193",
    year = "2021"
}

@article{Eguchi:1976db,
      author         = "Eguchi, Tohru and Freund, Peter G. O.",
      title          = "{Quantum Gravity and World Topology}",
      journal        = "Phys. Rev. Lett.",
      volume         = "37",
      year           = "1976",
      pages          = "1251",
      doi            = "10.1103/PhysRevLett.37.1251",
      reportNumber   = "EFI 76/52-CHICAGO",
      SLACcitation   = "%%CITATION = PRLTA,37,1251;%%"
}


@article{Delbourgo:1972xb,
      author         = "Delbourgo, Robert and Salam, Abdus",
      title          = "{The gravitational correction to pcac}",
      journal        = "Phys. Lett.",
      volume         = "40B",
      year           = "1972",
      pages          = "381-382",
      doi            = "10.1016/0370-2693(72)90825-8",
      reportNumber   = "ICTP-71-24",
      SLACcitation   = "%%CITATION = PHLTA,40B,381;%%"
}

@article{AlvarezGaume:1983ig,
      author         = "Alvarez-Gaume, Luis and Witten, Edward",
      title          = "{Gravitational Anomalies}",
      journal        = "Nucl. Phys.",
      volume         = "B234",
      year           = "1984",
      pages          = "269",
      doi            = "10.1016/0550-3213(84)90066-X",
      reportNumber   = "HUTP-83/A039",
      SLACcitation   = "%%CITATION = NUPHA,B234,269;%%"
}



@article{Dowker:1977tp,
      author         = "Dowker, J. S.",
      title          = "{Another Discussion of the Axial Vector Anomaly and the
                        Index Theorem}",
      journal        = "J. Phys.",
      volume         = "A11",
      year           = "1978",
      pages          = "347",
      doi            = "10.1088/0305-4470/11/2/012",
      reportNumber   = "PRINT-78-0053 (MANCHESTER), C77-08-31-1",
      SLACcitation   = "%%CITATION = JPAGA,A11,347;%%"
}



@article{Chung:1998zb,
    author = "Chung, Daniel J. H. and Kolb, Edward W. and Riotto, Antonio",
    title = "{Superheavy dark matter}",
    eprint = "hep-ph/9802238",
    archivePrefix = "arXiv",
    reportNumber = "FERMILAB-PUB-98-021-A, CERN-TH-98-37, OUTP-98-02-P, FERMILAB-FERMILAB-PUB-98-021-A, CERN-CERN-TH-98-37, OXFORD-U. --OUTP-98-02-P",
    doi = "10.1103/PhysRevD.59.023501",
    journal = "Phys. Rev. D",
    volume = "59",
    pages = "023501",
    year = "1998"
}

@article{Clery:2021bwz,
    author = "Clery, Simon and Mambrini, Yann and Olive, Keith A. and Verner, Sarunas",
    title = "{Gravitational portals in the early Universe}",
    eprint = "2112.15214",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "UMN-TH-4110/22, FTPI-MINN-22/02, CERN-TH-2021-222",
    doi = "10.1103/PhysRevD.105.075005",
    journal = "Phys. Rev. D",
    volume = "105",
    number = "7",
    pages = "075005",
    year = "2022"
}

@article{Bernal:2018qlk,
    author = "Bernal, Nicol\'as and Dutra, Ma\'\i{}ra and Mambrini, Yann and Olive, Keith and Peloso, Marco and Pierre, Mathias",
    title = "{Spin-2 Portal Dark Matter}",
    eprint = "1803.01866",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevD.97.115020",
    journal = "Phys. Rev. D",
    volume = "97",
    number = "11",
    pages = "115020",
    year = "2018"
}

@article{Kolb:2023ydq,
    author = "Kolb, Edward W. and Long, Andrew J.",
    title = "{Cosmological gravitational particle production and its implications for cosmological relics}",
    eprint = "2312.09042",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    journal = "",
    month = "12",
    year = "2023"
}

@article{Maleknejad:2022gyf,
    author = "Maleknejad, Azadeh and McDonough, Evan",
    title = "{Ultralight pion and superheavy baryon dark matter}",
    eprint = "2205.12983",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CERN-TH-2022-086",
    doi = "10.1103/PhysRevD.106.095011",
    journal = "Phys. Rev. D",
    volume = "106",
    number = "9",
    pages = "095011",
    year = "2022"
}


@article{Kolb:2017jvz,
    author = "Kolb, Edward W. and Long, Andrew J.",
    title = "{Superheavy dark matter through Higgs portal operators}",
    eprint = "1708.04293",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.96.103540",
    journal = "Phys. Rev. D",
    volume = "96",
    number = "10",
    pages = "103540",
    year = "2017"
}


@article{Ema:2019yrd,
    author = "Ema, Yohei and Nakayama, Kazunori and Tang, Yong",
    title = "{Production of purely gravitational dark matter: the case of fermion and vector boson}",
    eprint = "1903.10973",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "DESY-19-050, DESY 19-050, KEK-TH-2114, UT-19-04",
    doi = "10.1007/JHEP07(2019)060",
    journal = "JHEP",
    volume = "07",
    pages = "060",
    year = "2019"
}


@article{Greene:1998nh,
    author = "Greene, Patrick B. and Kofman, Lev",
    title = "{Preheating of fermions}",
    eprint = "hep-ph/9807339",
    archivePrefix = "arXiv",
    reportNumber = "UH-IFA-98-44",
    doi = "10.1016/S0370-2693(99)00020-9",
    journal = "Phys. Lett. B",
    volume = "448",
    pages = "6--12",
    year = "1999"
}


@article{Adshead:2018oaa,
    author = "Adshead, Peter and Pearce, Lauren and Peloso, Marco and Roberts, Michael A. and Sorbo, Lorenzo",
    title = "{Phenomenology of fermion production during axion inflation}",
    eprint = "1803.04501",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1088/1475-7516/2018/06/020",
    journal = "JCAP",
    volume = "06",
    pages = "020",
    year = "2018"
}


@article{Maleknejad:2019hdr,
    author = "Maleknejad, Azadeh",
    title = "{Dark Fermions and Spontaneous $CP$ violation in $SU(2)$-axion Inflation}",
    eprint = "1909.11545",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP07(2020)154",
    journal = "JHEP",
    volume = "07",
    pages = "154",
    year = "2020"
}


@article{Maleknejad:2020yys,
    author = "Maleknejad, Azadeh",
    title = "{SU(2)R and its axion in cosmology: A common origin for inflation, cold sterile neutrinos, and baryogenesis}",
    eprint = "2012.11516",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CERN-TH-2020-217",
    doi = "10.1103/PhysRevD.104.083518",
    journal = "Phys. Rev. D",
    volume = "104",
    number = "8",
    pages = "083518",
    year = "2021"
}


@article{Maleknejad:2020pec,
    author = "Maleknejad, Azadeh",
    title = "{Chiral anomaly in SU(2)$_{R}$-axion inflation and the new prediction for particle cosmology}",
    eprint = "2103.14611",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CERN-TH-2021-034",
    doi = "10.1007/JHEP06(2021)113",
    journal = "JHEP",
    volume = "21",
    pages = "113",
    year = "2020"
}


@article{Alexander:2004us,
    author = "Alexander, Stephon Haigh-Solom and Peskin, Michael E. and Sheikh-Jabbari, Mohammad M.",
    title = "{Leptogenesis from gravity waves in models of inflation}",
    eprint = "hep-th/0403069",
    archivePrefix = "arXiv",
    reportNumber = "SLAC-PUB-10226, SU-ITP-04-08",
    doi = "10.1103/PhysRevLett.96.081301",
    journal = "Phys. Rev. Lett.",
    volume = "96",
    pages = "081301",
    year = "2006"
}




@article{Maldacena:2002vr,
    author = "Maldacena, Juan Martin",
    title = "{Non-Gaussian features of primordial fluctuations in single field inflationary models}",
    eprint = "astro-ph/0210603",
    archivePrefix = "arXiv",
    doi = "10.1088/1126-6708/2003/05/013",
    journal = "JHEP",
    volume = "05",
    pages = "013",
    year = "2003"
}
@article{JHEP,
    author = "Maleknejad, Azadeh and Kopp, Joachim",
    title = "{Weyl Fermion Creation by Cosmological Gravitational Wave Background at 1-Loop}",
    eprint = "	arXiv:2406.01534"
}

@article{Garny:2015sjg,
    author = "Garny, Mathias and Sandora, McCullen and Sloth, Martin S.",
    title = "{Planckian Interacting Massive Particles as Dark Matter}",
    eprint = "1511.03278",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CERN-PH-TH-2015-264",
    doi = "10.1103/PhysRevLett.116.101302",
    journal = "Phys. Rev. Lett.",
    volume = "116",
    number = "10",
    pages = "101302",
    year = "2016"
}

@article{in-preparation-I,
    author = "Roper Pol, Alberto and Maleknejad, Azadeh and Kopp, Joachim",
    title = "{Simulating Fermion Production by Gravitational Waves Background}",
    year = "2024",
    journal = "",
    note = "in preparation",
}

@article{in-preparation-II,
    author = "Bagherian, Hengameh and Maleknejad, Azadeh",
    title = "{Weyl Fermions and Gravitational Waves in Inflation}",
    year = "2024",
    journal = "",
    note = "in preparation",
}

@article{Evans:2021gyd,
    author = "Evans, Matthew and others",
    title = "{A Horizon Study for Cosmic Explorer: Science, Observatories, and Community}",
    eprint = "2109.09882",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.IM",
    reportNumber = "CE-P2100003-v7, Cosmic Explorer technical report CE-P2100003-v6",
    journal = "",
    month = "9",
    year = "2021"
}

@article{Adshead:2015jza,
    author = "Adshead, Peter and Sfakianakis, Evangelos I.",
    title = "{Leptogenesis from left-handed neutrino production during axion inflation}",
    eprint = "1508.00881",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1103/PhysRevLett.116.091301",
    journal = "Phys. Rev. Lett.",
    volume = "116",
    number = "9",
    pages = "091301",
    year = "2016"
}

@article{Maggiore:2019uih,
    author = "Maggiore, Michele and others",
    title = "{Science Case for the Einstein Telescope}",
    eprint = "1912.02622",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1088/1475-7516/2020/03/050",
    journal = "JCAP",
    volume = "03",
    pages = "050",
    year = "2020"
}




@book{Strominger:2017zoo,
    author = "Strominger, Andrew",
    title = "{Lectures on the Infrared Structure of Gravity and Gauge Theory}",
    eprint = "1703.05448",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    isbn = "978-0-691-17973-5",
    month = "3",
    year = "2017"
}

@article{Alvarez-Gaume:1983ihn,
    author = "Alvarez-Gaume, Luis and Witten, Edward",
    editor = "Salam, A. and Sezgin, E.",
    title = "{Gravitational Anomalies}",
    reportNumber = "HUTP-83/A039",
    doi = "10.1016/0550-3213(84)90066-X",
    journal = "Nucl. Phys. B",
    volume = "234",
    pages = "269",
    year = "1984"
}




@article{Witten:1984rs,
    author = "Witten, Edward",
    title = "{Cosmic Separation of Phases}",
    reportNumber = "PRINT-84-0400 (IAS,PRINCETON)",
    doi = "10.1103/PhysRevD.30.272",
    journal = "Phys. Rev. D",
    volume = "30",
    pages = "272--285",
    year = "1984"
}


@article{Schwaller:2015tja,
    author = "Schwaller, Pedro",
    title = "{Gravitational Waves from a Dark Phase Transition}",
    eprint = "1504.07263",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CERN-PH-TH-2015-093",
    doi = "10.1103/PhysRevLett.115.181101",
    journal = "Phys. Rev. Lett.",
    volume = "115",
    number = "18",
    pages = "181101",
    year = "2015"
}


@article{Caprini:2015zlo,
    author = "Caprini, Chiara and others",
    title = "{Science with the space-based interferometer eLISA. II: Gravitational waves from cosmological phase transitions}",
    eprint = "1512.06239",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "DESY-15-246",
    doi = "10.1088/1475-7516/2016/04/001",
    journal = "JCAP",
    volume = "04",
    pages = "001",
    year = "2016"
}


@article{RoperPol:2023bqa,
    author = "Roper Pol, A. and Neronov, A. and Caprini, C. and Boyer, T. and Semikoz, D.",
    title = "{LISA and $\gamma$-ray telescopes as multi-messenger probes of a first-order cosmological phase transition}",
    eprint = "2307.10744",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    journal = "",
    month = "7",
    year = "2023"
}


@article{Brandenburg:2021aln,
    author = "Brandenburg, Axel and He, Yutong and Kahniashvili, Tina and Rheinhardt, Matthias and Schober, Jennifer",
    title = "{Relic gravitational waves from the chiral magnetic effect}",
    eprint = "2101.08178",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "NORDITA-2021-005",
    doi = "10.3847/1538-4357/abe4d7",
    journal = "Astrophys. J.",
    volume = "911",
    number = "2",
    pages = "110",
    year = "2021"
}


@article{RoperPol:2021xnd,
    author = "Roper Pol, Alberto and Mandal, Sayan and Brandenburg, Axel and Kahniashvili, Tina",
    title = "{Polarization of gravitational waves from helical MHD turbulent sources}",
    eprint = "2107.05356",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    reportNumber = "NORDITA-2021-062",
    doi = "10.1088/1475-7516/2022/04/019",
    journal = "JCAP",
    volume = "04",
    number = "04",
    pages = "019",
    year = "2022"
}


@article{Adshead:2019igv,
    author = "Adshead, Peter and Giblin, John T. and Pieroni, Mauro and Weiner, Zachary J.",
    title = "{Constraining Axion Inflation with Gravitational Waves across 29 Decades in Frequency}",
    eprint = "1909.12843",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevLett.124.171301",
    journal = "Phys. Rev. Lett.",
    volume = "124",
    number = "17",
    pages = "171301",
    year = "2020"
}


@article{Figueroa:2022iho,
    author = "Figueroa, Daniel G. and Florio, Adrien and Loayza, Nicolas and Pieroni, Mauro",
    title = "{Spectroscopy of particle couplings with gravitational waves}",
    eprint = "2202.05805",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.106.063522",
    journal = "Phys. Rev. D",
    volume = "106",
    number = "6",
    pages = "063522",
    year = "2022"
}


@article{Hindmarsh:1994re,
    author = "Hindmarsh, M. B. and Kibble, T. W. B.",
    title = "{Cosmic strings}",
    eprint = "hep-ph/9411342",
    archivePrefix = "arXiv",
    reportNumber = "SUSX-TP-94-74, IMPERIAL-TP-94-95-5, NI-94025",
    doi = "10.1088/0034-4885/58/5/001",
    journal = "Rept. Prog. Phys.",
    volume = "58",
    pages = "477--562",
    year = "1995"
}


@article{Auclair:2019wcv,
    author = "Auclair, Pierre and others",
    title = "{Probing the gravitational wave background from cosmic strings with LISA}",
    eprint = "1909.00819",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1088/1475-7516/2020/04/034",
    journal = "JCAP",
    volume = "04",
    pages = "034",
    year = "2020"
}

@article{Caprini:2009fx,
    author = "Caprini, Chiara and Durrer, Ruth and Konstandin, Thomas and Servant, Geraldine",
    title = "{General Properties of the Gravitational Wave Spectrum from Phase Transitions}",
    eprint = "0901.1661",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.79.083519",
    journal = "Phys. Rev. D",
    volume = "79",
    pages = "083519",
    year = "2009"
}


@article{Caprini:2009yp,
    author = "Caprini, Chiara and Durrer, Ruth and Servant, Geraldine",
    title = "{The stochastic gravitational wave background from turbulence and magnetic fields generated by a first-order phase transition}",
    eprint = "0909.0622",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1088/1475-7516/2009/12/024",
    journal = "JCAP",
    volume = "12",
    pages = "024",
    year = "2009"
}


@book{Scully_Zubairy_1997,
    author = "Scully, Marlan O. and Zubairy, M. Suhail",
    title = "{Quantum Optics}",
    isbn = "978-0-19-852682-7",
    year = "1997"
}

@article{Breitbach:2018ddu,
    author = "Breitbach, Moritz and Kopp, Joachim and Madge, Eric and Opferkuch, Toby and Schwaller, Pedro",
    title = "{Dark, Cold, and Noisy: Constraining Secluded Hidden Sectors with Gravitational Waves}",
    eprint = "1811.11175",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    reportNumber = "CERN-TH-2018-255, MITP/18-115",
    doi = "10.1088/1475-7516/2019/07/007",
    journal = "JCAP",
    volume = "07",
    pages = "007",
    year = "2019"
}

@mastersthesis{Breitbach:2018kma,
    author = "Breitbach, Moritz",
    title = "{Gravitational Waves from Cosmological Phase Transitions}",
    eprint = "2204.09661",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    school = "Mainz U.",
    year = "2018"
} 
@article{Durrer:2010xc,
    author = "Durrer, Ruth",
   editor = "Basilakos, Spyros and Cadoni, Mariano and Cavaglia, Marco and Christodoulakis, Theodosios and Vagenas, Elias C.",
   title = "{Gravitational waves from cosmological phase transitions}",
    eprint = "1002.1389",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1088/1742-6596/222/1/012021",
    journal = "J. Phys. Conf. Ser.",
    volume = "222",
    pages = "012021",
    year = "2010"
}


@article{Caprini:2018mtu,
    author = "Caprini, Chiara and Figueroa, Daniel G.",
    title = "{Cosmological Backgrounds of Gravitational Waves}",
    eprint = "1801.04268",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1088/1361-6382/aac608",
    journal = "Class. Quant. Grav.",
    volume = "35",
    number = "16",
    pages = "163001",
    year = "2018"
}


@article{RoperPol:2022iel,
    author = "Roper Pol, Alberto and Caprini, Chiara and Neronov, Andrii and Semikoz, Dmitri",
    title = "{Gravitational wave signal from primordial magnetic fields in the Pulsar Timing Array frequency band}",
    eprint = "2201.05630",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1103/PhysRevD.105.123502",
    journal = "Phys. Rev. D",
    volume = "105",
    number = "12",
    pages = "123502",
    year = "2022"
}


@book{Weinberg:2008zzc,
    author = "Weinberg, Steven",
    title = "{Cosmology}",
    isbn = "978-0-19-852682-7",
    year = "2008"
}


@article{Weinberg:2005vy,
    author = "Weinberg, Steven",
    title = "{Quantum contributions to cosmological correlations}",
    eprint = "hep-th/0506236",
    archivePrefix = "arXiv",
    reportNumber = "UTTG-01-05",
    doi = "10.1103/PhysRevD.72.043514",
    journal = "Phys. Rev. D",
    volume = "72",
    pages = "043514",
    year = "2005"
}


@article{Green:2023ids,
    author = "Green, Daniel and Huang, Yiwen and Shen, Chia-Hsien and Baumann, Daniel",
    title = "{Positivity from Cosmological Correlators}",
    eprint = "2310.02490",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "10",
    year = "2023"
}


@article{Senatore:2012nq,
    author = "Senatore, Leonardo and Zaldarriaga, Matias",
    title = "{On Loops in Inflation II: IR Effects in Single Clock Inflation}",
    eprint = "1203.6354",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "SLAC-PUB-15860",
    doi = "10.1007/JHEP01(2013)109",
    journal = "JHEP",
    volume = "01",
    pages = "109",
    year = "2013"
}

@book{Maggiore:2007ulw,
    author = "Maggiore, Michele",
    title = "{Gravitational Waves. Vol. 1: Theory and Experiments}",
    doi = "10.1093/acprof:oso/9780198570745.001.0001",
    isbn = "978-0-19-171766-6, 978-0-19-852074-0",
    publisher = "Oxford University Press",
    year = "2007"
}

@book{Maggiore:2018sht,
    author = "Maggiore, Michele",
    title = "{Gravitational Waves. Vol. 2: Astrophysics and Cosmology}",
    isbn = "978-0-19-857089-9",
    publisher = "Oxford University Press",
    month = "3",
    year = "2018"
}

@article{Sorbo:2011rz,
    author = "Sorbo, Lorenzo",
    title = "{Parity violation in the Cosmic Microwave Background from a pseudoscalar inflaton}",
    eprint = "1101.1525",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1088/1475-7516/2011/06/003",
    journal = "JCAP",
    volume = "06",
    pages = "003",
    year = "2011"
}



@article{Maleknejad:2016qjz,
    author = "Maleknejad, Azadeh",
    title = "{Axion Inflation with an SU(2) Gauge Field: Detectable Chiral Gravity Waves}",
    eprint = "1604.03327",
    archivePrefix = "arXiv",
    primaryClass = "hep-ph",
    doi = "10.1007/JHEP07(2016)104",
    journal = "JHEP",
    volume = "07",
    pages = "104",
    year = "2016"
}

@book{Schwartz:2014sze,
    author = "Schwartz, Matthew D.",
    title = "{Quantum Field Theory and the Standard Model}",
    isbn = "978-1-107-03473-0, 978-1-107-03473-0",
    publisher = "Cambridge University Press",
    month = "3",
    year = "2014"
}

@book{Parker_Toms_2009, place={Cambridge}, series={Cambridge Monographs on Mathematical Physics}, title={Quantum Field Theory in Curved Spacetime: Quantized Fields and Gravity}, publisher={Cambridge University Press}, author={Parker, Leonard and Toms, David}, year={2009}, collection={Cambridge Monographs on Mathematical Physics}}

@article{Chung:2011ck,
    author = "Chung, Daniel J. H. and Everett, Lisa L. and Yoo, Hojin and Zhou, Peng",
    title = "{Gravitational Fermion Production in Inflationary Cosmology}",
    eprint = "1109.2524",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    doi = "10.1016/j.physletb.2012.04.066",
    journal = "Phys. Lett. B",
    volume = "712",
    pages = "147--154",
    year = "2012"
}

@article{Aggarwal:2020olq,
    author = "Aggarwal, Nancy and others",
    title = "{Challenges and opportunities of gravitational-wave searches at MHz to GHz frequencies}",
    eprint = "2011.12414",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    reportNumber = "CERN-TH-2020-185, HIP-2020-28/TH, DESY 20-195, CERN-TH-2020-185, HIP-2020-28/TH, DESY 20-195",
    doi = "10.1007/s41114-021-00032-5",
    journal = "Living Rev. Rel.",
    volume = "24",
    number = "1",
    pages = "4",
    year = "2021"
}

@article{LISACosmologyWorkingGroup:2022jok,
    author = "Auclair, Pierre and others",
    collaboration = "LISA Cosmology Working Group",
    title = "{Cosmology with the Laser Interferometer Space Antenna}",
    eprint = "2204.05434",
    archivePrefix = "arXiv",
    primaryClass = "astro-ph.CO",
    reportNumber = "LISA CosWG-22-03, FERMILAB-PUB-22-349-SCD",
    doi = "10.1007/s41114-023-00045-2",
    journal = "Living Rev. Rel.",
    volume = "26",
    number = "1",
    pages = "5",
    year = "2023"
}


